Robotic Playing for Hierarchical Complex Skill Learning

In complex manipulation scenarios (e.g. tasks requiring complex interaction of two hands or in-hand manipulation), generalization is a hard problem. Current methods still either require a substantial amount of (supervised) training data and / or strong assumptions on both the environment and the task. In this paradigm, controllers solving these tasks tend to be complex. We propose a paradigm of maintaining simpler controllers solving the task in a small number of specific situations. In order to generalize to novel situations, the robot transforms the environment from novel situations into a situation where the solution of the task is already known. Our solution to this problem is to play with objects and use previously trained skills (basis skills). These skills can either be used for estimating or for changing the current state of the environment and are organized in skill hierarchies. The approach is evaluated in complex pick-and-place scenarios that involve complex manipulation. We further show that these skills can be learned by autonomous playing.

==> ecm.tex <==
\begin{figure*}[t!]
\centering
  \scalebox{0.65} {
\begin{tikzpicture}[every node/.style = {shape=rectangle, rounded corners},>=stealth',bend angle=45, auto]

  \tikzstyle{place}=[circle,thick,draw=blue!75,fill=blue!20,minimum size=6mm]

  \begin{scope}
  
  	\draw(1,2.1) node[rectangle, minimum width=3cm, minimum height=1.5cm,draw] (i1) {$I_{\mathrm{sp}} \equiv$ Speech recognition};
  	\draw(9,2.1) node[rectangle, minimum width=3cm, minimum height=1.5cm,draw] (i2) {$I_{\mathrm{kb}} \equiv$ Keyboard input};
  	
  	\node[text width=2cm,align=left] at (-9,2.1) {Layer 1 $\equiv$ Input coupler};
  	\node[text width=5cm,align=left] at (-7.5,0) {Layer 2 $\equiv$ Desired complex action percepts};
  	\node[text width=5cm,align=left] at (-7.5,-2) {Layer 3 $\equiv$ Sensing\\ actions};
  	\node[text width=5cm,align=left] at (-7.5,-4) {Layer 4 $\equiv$ \\ Perceptual\\ states};
  	\node[text width=5cm,align=left] at (-7.5,-7) {Layer 5 $\equiv$ \\ Preparatory\\ skills};
  	\draw[dashed](-8.8,1) -- (18,1);
                
    \draw(-1.5,0) node[ellipse, minimum height=1.3cm,draw] (c1) {$P_1 \equiv $ Complex Skill 1};
    \draw(11,0) node[ellipse, minimum height=1.3cm,draw] (c2) {$P_2 \equiv $ Complex Skill 2};
    
    \draw[dashed](-8.8,-1) -- (18,-1);
    
    \draw(-6,-2) node[circle, minimum size=1cm,draw] (s11) {$S_1$};
    \draw(-2.5,-2) node[circle, minimum size=1cm,draw] (s21) {$S_2$};
    \draw(1.5,-2) node[circle, minimum size=1cm,draw] (sdot1) {$\dots$};
    \draw(4.5,-2) node[circle, minimum size=1cm,draw] (sn1) {$S_N$};
    
    \draw(7.5,-2) node[circle, minimum size=1cm,draw] (s12) {$S_1$};
    \draw(11,-2) node[circle, minimum size=1cm,draw] (sdot2) {$\dots$};
    \draw(14.5,-2) node[circle, minimum size=1cm,draw] (sn2) {$S_N$};
    
    \path[->] (c1) edge [line width=0.4mm] node {} (s11.north);
    \path[->] (c1) edge [line width=0.4mm] node {} (s21.north);
    \path[->] (c1) edge [line width=0.4mm] node {} (sdot1.north);
    \path[->] (c1) edge [line width=0.4mm] node {} (sn1.north);
    
    \path[->] (c2) edge [line width=0.4mm] node {} (s12.north);
    \path[->] (c2) edge [line width=0.4mm] node {} (sdot2.north);
    \path[->] (c2) edge [line width=0.4mm] node {} (sn2.north);
    
    \draw[dashed](-8.8,-3) -- (18,-3);
    
    \draw(-7.5,-4) node[circle, minimum size=1.2cm, inner sep=0pt,draw] (e111) {$E^{P_1}_{1S_1}$};
    \draw(-6,-4) node[circle, minimum size=1.2cm, inner sep=0pt,draw] (edot11) {$E^{P_1}_{\dots S_1}$};
    \draw(-4.5,-4) node[circle, minimum size=1.2cm, inner sep=0pt,draw] (el11) {$E^{P_1}_{L_{1,1}S_1}$};
    
    \draw(-3,-4) node[circle, minimum size=1.2cm, inner sep=0pt,draw] (e121) {$E^{P_1}_{1S_2}$};
    \draw(-1.5,-4) node[circle, minimum size=1.2cm, inner sep=0pt,draw] (edot21) {$E^{P_1}_{\dots S_2}$};
    \draw(0,-4) node[circle, minimum size=1.2cm, inner sep=0pt,draw] (el21) {$E^{P_1}_{L_{1,2}S_2}$};
    
    \draw(1.5,-4) node[circle, minimum size=1.2cm, inner sep=0pt,draw] (edotdot1) {$\dots$};
    
    \draw(3,-4) node[circle, minimum size=1.2cm, inner sep=0pt,draw] (e1n1) {$E^{P_1}_{1S_N}$};
    \draw(4.5,-4) node[circle, minimum size=1.2cm, inner sep=0pt,draw] (edotn1) {$E^{P_1}_{\dots S_N}$};
    \draw(6,-4) node[circle, minimum size=1.2cm, inner sep=0pt,draw] (eln1) {$E^{P_1}_{L_{1,N}S_N}$};
    
    \draw(7.5,-4) node[circle, minimum size=1.2cm, inner sep=0pt,draw] (e112) {$E^{P_2}_{1S_1}$};
    \draw(9,-4) node[circle, minimum size=1.2cm, inner sep=0pt,draw] (edot12) {$E^{P_2}_{\dots S_1}$};
    \draw(10.5,-4) node[circle, minimum size=1.2cm, inner sep=0pt,draw] (el12) {$E^{P_2}_{L_{2,1}S_1}$};
    
    \draw(12,-4) node[circle, minimum size=1.2cm, inner sep=0pt,draw] (edotdot2) {$\dots$};
    
    \draw(13.5,-4) node[circle, minimum size=1.2cm, inner sep=0pt,draw] (e1n2) {$E^{P_2}_{1S_N}$};
    \draw(15,-4) node[circle, minimum size=1.2cm, inner sep=0pt,draw] (edotn2) {$E^{P_2}_{\dots S_1}$};
    \draw(16.5,-4) node[circle, minimum size=1.2cm, inner sep=0pt,draw] (eln2) {$E^{P_2}_{L_{2,N}S_N}$};
    
    \draw[dashed](-8.8,-5.5) -- (18,-5.5);
    
    \draw(-5,-7) node[rectangle, minimum width=3cm, minimum height=1.5cm, color=red, draw] (atocp2) {};
    \draw(15,-7) node[rectangle, minimum width=3cm, minimum height=1.5cm, color=red, draw] (atocp1) {};
    
    \draw(0,-7) node[rectangle, minimum width=3cm, minimum height=1.5cm,draw] (a1) {$A_1 \equiv$ Preparatory skill 1};
    \draw(5,-7) node[rectangle, minimum width=3cm, minimum height=1.5cm,draw] (a2) {$\dots$};
    \draw(10,-7) node[rectangle, minimum width=3cm, minimum height=1.5cm,draw] (a3) {$A_M \equiv$ Preparatory skill $M$};
    
	\path[->] (i1) edge [line width=0.2mm] node {} (c1.north);
	\path[->] (i1) edge [line width=0.2mm] node {} (c2.north);
	\path[->] (i2) edge [line width=0.2mm] node {} (c1.north);
	\path[->] (i2) edge [line width=0.2mm] node {} (c2.north);
    
    \path[->] (s11) edge [line width=0.4mm] node {} (e111.north);
    \path[->] (s11) edge [line width=0.4mm] node {} (edot11.north);
    \path[->] (s11) edge [line width=0.4mm] node {} (el11.north);
    
    \path[->] (s21) edge [line width=0.4mm] node {} (e121.north);
    \path[->] (s21) edge [line width=0.4mm] node {} (edot21.north);
    \path[->] (s21) edge [line width=0.4mm] node {} (el21.north);
    
    \path[->] (sn1) edge [line width=0.4mm] node {} (e1n1.north);
    \path[->] (sn1) edge [line width=0.4mm] node {} (edotn1.north);
    \path[->] (sn1) edge [line width=0.4mm] node {} (eln1.north);
    
    \path[->] (sdot1) edge [line width=0.4mm] node {} (edotdot1.north);
    
    \path[->] (s12) edge [line width=0.4mm] node {} (e112.north);
    \path[->] (s12) edge [line width=0.4mm] node {} (edot12.north);
    \path[->] (s12) edge [line width=0.4mm] node {} (el12.north);
    
    \path[->] (sn2) edge [line width=0.4mm] node {} (e1n2.north);
    \path[->] (sn2) edge [line width=0.4mm] node {} (edotn2.north);
    \path[->] (sn2) edge [line width=0.4mm] node {} (eln2.north);
    
    \path[->] (sdot2.south) edge [line width=0.4mm] node {} (edotdot2.north);
    
	\path[->] (e111.south) [color=red] edge node {} (atocp2.north);
    \path[->] (edot11.south) [color=red] edge node {} (atocp2.north);
    \path[->] (el11.south) [color=red] edge node {} (atocp2.north);
    \path[->] (e121.south) [color=red] edge node {} (atocp2.north);
    \path[->] (edot21.south) [color=red] edge node {} (atocp2.north);
    \path[->] (el21.south) [color=red] edge node {} (atocp2.north);
    \path[->] (e1n1.south) [color=red] edge node {} (atocp2.north);
    \path[->] (edotn1.south) [color=red] edge node {} (atocp2.north);
    \path[->] (eln1.south) [color=red] edge node {} (atocp2.north);
    \path[->] (edotdot1.south) [color=red] edge node {} (atocp2.north);
    
    \path[->] (e112.south) [color=red] edge  node {} (atocp1.north);
    \path[->] (edot12.south) [color=red] edge  node {} (atocp1.north);
    \path[->] (el12.south) [color=red] edge  node {} (atocp1.north);
    \path[->] (e1n2.south) [color=red] edge  node {} (atocp1.north);
    \path[->] (edotn2.south) [color=red] edge  node {} (atocp1.north);
    \path[->] (eln2.south) [color=red] edge  node {} (atocp1.north);
    \path[->] (edotdot2.south) [color=red] edge  node {} (atocp1.north);
    
    \node[dummy] (dummy2a) [left of = atocp2, xshift = -2.5cm] {};
    \node[dummy] (dummy2b) [above of = dummy2a, yshift = 6.9cm] {};
    \node[dummy] (dummy2c) [right of = dummy2b, xshift = 9.5cm] {};
    \path[-] (atocp2.west) [color=red] edge  node {} (dummy2a.east);
    \path[-] (dummy2a.north) [color=red] edge  node {} (dummy2b.south);
    \path[-] (dummy2b.east) [color=red] edge  node {} (dummy2c.west);
    \path[->] (dummy2c.east) [color=red] edge  node {} (c2.west);
    
    \node[dummy] (dummy1a) [left of = atocp1, xshift = 3.5cm] {};
    \node[dummy] (dummy1b) [above of = dummy1a, yshift = 6.9cm] {};
    \node[dummy] (dummy1c) [right of = dummy1b, xshift = -9.5cm] {};
    \path[-] (atocp1.east) [color=red] edge  node {} (dummy1a.west);
    \path[-] (dummy1a.north) [color=red] edge  node {} (dummy1b.south);
    \path[-] (dummy1b.west) [color=red] edge  node {} (dummy1c.east);
    \path[->] (dummy1c.west) [color=red] edge  node {} (c1.east);
    
    \path[->] (e111.south) edge node {} (a1.north);
    \path[->] (edot11.south) edge node {} (a1.north);
    \path[->] (el11.south) edge node {} (a1.north);
    \path[->] (e121.south) edge node {} (a1.north);
    \path[->] (edot21.south) edge node {} (a1.north);
    \path[->] (el21.south) edge node {} (a1.north);
    \path[->] (e1n1.south) edge node {} (a1.north);
    \path[->] (edotn1.south) edge node {} (a1.north);
    \path[->] (eln1.south) edge node {} (a1.north);
    \path[->] (edotdot1.south) edge node {} (a1.north);
    \path[->] (e112.south) edge  node {} (a1.north);
    \path[->] (edot12.south) edge  node {} (a1.north);
    \path[->] (el12.south) edge  node {} (a1.north);
    \path[->] (e1n2.south) edge  node {} (a1.north);
    \path[->] (edotn2.south) edge  node {} (a1.north);
    \path[->] (eln2.south) edge  node {} (a1.north);
    \path[->] (edotdot2.south) edge  node {} (a1.north);
    
    \path[->] (e111.south) edge  node {} (a2.north);
    \path[->] (edot11.south) edge  node {} (a2.north);
    \path[->] (el11.south) edge  node {} (a2.north);
    \path[->] (e121.south) edge  node {} (a2.north);
    \path[->] (edot21.south) edge  node {} (a2.north);
    \path[->] (el21.south) edge  node {} (a2.north);
    \path[->] (e1n1.south) edge  node {} (a2.north);
    \path[->] (edotn1.south) edge  node {} (a2.north);
    \path[->] (eln1.south) edge  node {} (a2.north);
    \path[->] (edotdot1.south) edge  node {} (a2.north);
    \path[->] (e112.south) edge  node {} (a2.north);
    \path[->] (edot12.south) edge  node {} (a2.north);
    \path[->] (el12.south) edge  node {} (a2.north);
    \path[->] (e1n2.south) edge  node {} (a2.north);
    \path[->] (edotn2.south) edge  node {} (a2.north);
    \path[->] (eln2.south) edge  node {} (a2.north);
    \path[->] (edotdot2.south) edge  node {} (a2.north);
    
    \path[->] (e111.south) edge  node {} (a3.north);
    \path[->] (edot11.south) edge  node {} (a3.north);
    \path[->] (el11.south) edge  node {} (a3.north);
    \path[->] (e121.south) edge  node {} (a3.north);
    \path[->] (edot21.south) edge  node {} (a3.north);
    \path[->] (el21.south) edge  node {} (a3.north);
    \path[->] (e1n1.south) edge  node {} (a3.north);
    \path[->] (edotn1.south) edge  node {} (a3.north);
    \path[->] (eln1.south) edge  node {} (a3.north);
    \path[->] (edotdot1.south) edge  node {} (a3.north);
    \path[->] (e112.south) edge  node {} (a3.north);
    \path[->] (edot12.south) edge  node {} (a3.north);
    \path[->] (el12.south) edge  node {} (a3.north);
    \path[->] (e1n2.south) edge  node {} (a3.north);
    \path[->] (edotn2.south) edge  node {} (a3.north);
    \path[->] (eln2.south) edge  node {} (a3.north);
    \path[->] (edotdot2.south) edge  node {} (a3.north);
    
  \end{scope}
\end{tikzpicture}
}
\caption{ECM for autonomous robotic playing\textcolor{red}{todo}}
\label{fig:ecmplaying}
\end{figure*}
